VANET Connectivity Analysis

Vehicular Ad Hoc Networks (VANETs) are a peculiar subclass of mobile ad hoc networks that raise a number of technical challenges, notably from the point of view of their mobility models. In this paper, we provide a thorough analysis of the connectivity of such networks by leveraging on well-known results of percolation theory. By means of simulations, we study the influence of a number of parameters, including vehicle density, proportion of equipped vehicles, and radio communication range. We also study the influence of traffic lights and roadside units. Our results provide insights on the behavior of connectivity. We believe this paper to be a valuable framework to assess the feasibility and performance of future applications relying on vehicular connectivity in urban scenarios.

==> Connectivity_adhoc-1.tex <==
\section{Vehicle-to-Vehicle Connectivity} \label{Sec:EvalConneAd-hocNet}

This section presents our findings on vehicle-to-vehicle (V2V) connectivity,
based on analysis and extensive experiments with microscopic vehicle mobility
simulation. We consider urban grids of two-lane bidirectional roads, in the
shape of Fig.~\ref{fig:domain}, with the number of horizontal and vertical
perpendicular roads ranging from $N=5$ to $10$. The entry and destination
points for vehicles are at the edges of the grid, as explained in
Sec.~\ref{Sec:Models}.

At first, we seek to understand how vehicles are distributed across the road
grid, as a function of their entrance rate and for each of the three above
mentioned settings. Our findings, detailed in
Sec.~\ref{sec:CarDensityfctCarFlow}, show that the presence and mode of
operation of traffic has a significant impact on the density and spatial
distribution of vehicles.

The differing vehicle placement conditions, as a result of the differing rates
of entrance (and exit) from the simulated road grid, influence the overall
connectivity and most notably the proportion of vehicles in the largest
cluster. Clearly, the highest the proportion, the more likely it is to have any
piece of information disseminated to all vehicles in the cluster. But, as it
will be explained in Sec.~\ref{sec:cluster}, traffic lights significantly
influence the size of largest cluster.

%%%% CAPTION
\begin{figure*}[htpb]
\includegraphics[width=\linewidth]{Merged_density_plots_anti-diametric.eps}
\caption{ } \label{fig:d}
\end{figure*}

On a different dimension of our investigation, we consider the critical range,
that is the minimum communication range that enables all vehicles to belong to
a single cluster. Again, traffic lights heavily influence the value of the
critical range Sec.\ref{sec:critical_range}. We shift gears in
Sec.~\ref{sec:market_penetration}, where we are concerned with vehicular
networks comprising a fraction of the circulating vehicles. Now, the presence
of vehicles that are not equipped with radios essentially model the spatial
distribution of the equipped vehicles and thus the vehicular network
connectivity.

\begin{table}[htb]
\caption{Simulation parameters} \small\addtolength{\tabcolsep}{-5pt}
\begin{tabular}{|l|l|}
\hline
Simulation interval & [0,999s] \\
\hline
Number of lane & 2  \\
\hline
Grid dimension & 5, 10 \\
\hline
Traffic lights regimes & Synchronized, Green Wave\\
\hline
Road segment length $L$ [m] & 400 \\
\hline
$f$ (CarArrival/h/lane) & 100..1500\\
\hline
Types of destination & Anti-Diametric, Random\\
\hline \hline
Connectivity range $r$ [m] & 100\\
\hline
\end{tabular}
\end{table}

Throughout this section, we present results for the three types of road traffic
control, as described in Sec.~\ref{Sec:Models}, differentiated by the existence
and operation of traffic lights: ``\textbf{N}o Traffic \textbf{L}ights''
(\textbf{NL}), ``\textbf{S}ynchronized Traffic \textbf{L}ights'' (\textbf{SL}),
and ``\textbf{G}reen \textbf{W}ave'' (\textbf{GW}). We combine those settings
with different road destination selection settings, again described in
Sec.~\ref{Sec:Models}: ``\textbf{A}nti-diametric'' or ``\textbf{R}andom''
destination road end points. For example, SL-R signifies synchronized traffic
lights with random destinations. Note that the green wave regime can be
meaningful when cars can keep a constant speed. This is not the case for the
random destination model, where cars are more likely to turn at intersections,
decelerate or even stop before doing so, and thus cause significant velocity
fluctuations; this is why we do not investigate the GW-R case.

\subsection{Vehicle Density} \label{sec:CarDensityfctCarFlow}

As the simulator allows us to control the in-flow rate for each source (entry)
point, we utilize this as the independent parameter in our experiments.
Nonetheless, the resultant placement of vehicles is what is of real interest.
This is why we investigate how the entrance rate (for a given $N$ dimension of
the road network grid) relates to the average vehicle density. We note
nonetheless that vehicle density, and their spatial distribution more
generally, do not depend only on the flow of cars entering the network but also
on the mobility regime and cars trip.

%% Make them smaller
\begin{figure*}[htpb]
\includegraphics[width=\linewidth]{Merged_density_plots_random.eps}
\caption{} \label{fig:d}
\end{figure*}

%%% Finalize references to all figures
First, for all figures, we observe that there is a variation of the
distribution across the road network. We differentiate \emph{peripheral road
segments} as those $4N$ segments between the vehicle entry and exit points and
the first-encountered intersection. We term all the remaining road segments in
the grid as \emph{central road segments}.

We first look at the scenarios with anti-diametric destinations and observe
that, as the vehicle in-flow rate increases, the vehicle density increases in a
similar manner for peripheral and central road segments. But this only up to a
certain value of $f$, e.g., $f=800$ for Fig.~\ref{fig:Car_density_Scenario1},
after which the density in central roads increases very slowly and then does
not increase any further. While, the vehicle density in peripheral roads
continue to increase beyond that point, until it also reaches a plateau, for a
larger in-flow rate, e.g., $f=1000$ for Fig.~\ref{fig:Car_density_Scenario1}.
This phenomenon occurs consistently for all scenarios, but with different
transition $f$ values. Basically, central road segment $\lambda$ is lower for
the GW compared to SL and NL. At the same time, the differentiation between
peripheral and central segments occurs for lower $f$ values for GW, compared to
those for SL and NL.

These variations are due to the role of traffic lights. Looking, for example,
at Fig.~\ref{fig:Car_density_Scenario3}, the central road density flattens at
$f=500$vehicles/h/lane. This is so, because traffic lights at the first
intersection encountered by vehicles, that is, at the limit of each peripheral
road segment, control the in-flow to the central road segments. Essentially,
they act as a bottleneck. At this point, traffic jams start building up at the
peripheral roads, up to the point the density reaches, at
$f=800$vehicles/h/lane, a plateau: the jammed peripheral roads do not allow the
entrance of more vehicles. In contrast, without traffic lights, stop signs at
intersections start acting as a bottleneck only when the amount of traffic is
such that long queues build up at all sides of the intersection. This
essentially ``shifts'' the saturation point for $\lambda$ to occur for
$f>1000$. But it is interesting to see that for NL, the plateau occurs for
peripheral and central roads for that same $f$. Again, peripheral roads reach
higher densities, up to the point they get jammed.

On the other hand, for scenarios with random destination(s), we also observe
the saturation phenomenon and the differentiation between peripheral and
central road segments (Fig.~\ref{fig:Car_density_Scenario4}). However, central
roads get more congested than peripheral roads. This peculiarity stems from the
trip type: with random destinations vehicle routes are longer while vehicles
are more likely to turn at intersections to reach their destination. As a
consequence, cars stay longer in the (simulated) road network and especially in
central road segments.

\subsection{Vehicle Clustering}\label{sec:cluster}

We study the clustering of cars both from an analytical and simulation
approach. For the scenario where we have simple intersections, we show that
accurate predictions of the network connectivity can be made using percolation
theory. For the scenarios involving traffic lights, we study connectivity using
our microscopic simulator and show the main differences with the simple
intersections case.   

\subsubsection{Analytical study}

For low vehicle arrival rates, road traffic has little impact on the
distribution of the cars along the roads. In the stationary regime, we can
model it with a spatial Poisson process. Also, we neglect the width of the
streets and associate them with lines. We obtain a one-dimensional process
along each road whose intensity  $\lambda$ is related to the car arrival rate
through the formula
$$
\lambda = \frac{2f}{\bar{v}},
$$
where $\bar{v}$ denotes the average speed of the cars. The factor $2$ is due to the bi-directionality of traffic.

Given the Poisson assumption, one can compute an upper bound on the average
fraction $E[\phi(t)]$ of cars that are connected to no other car in the
stationary regime, that is, when the road network is at a state that the rate
of vehicles entering the road network is the same as the rate of vehicle
leaving it:
$$
E[\phi(t)] = \exp(-2\lambda \rho r).
$$

Fig.~\ref{fig:isolated} shows a comparison of the analytical curve
with simulation results. The Poisson approximation shows its
limitations: when the density of cars is not very low, the
intersections start to shape their spatial distribution. Cars that
are stopped at an intersection are typically not isolated, whereas
cars leaving an intersection are well spaced and likely to be
isolated.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Isolated_cars.eps}
\caption{Theoretical and simulated fraction of isolated cars in a scenario with no traffic lights and Anti-diametric destinations. The size of the simulation domain is $N=10$ and road segments are $L=400m$ long.}
\label{fig:isolated}
\end{figure}

To compute the fraction of vehicles (nodes) belonging to the largest connected
component, we start by looking at the probability $p$ that a road segment (i.e.
the portion of road located between two consecutive intersections) is covered
by a sequence of connected cars. We can then see the network as an edge
percolation model, where each road segment is \emph{covered} (or \emph{open})
with probability $p$.

Percolation theory allows us to address the case where the network has an
infinite size, namely when $N\rightarrow\infty$. Then it is well known that
(see for example \cite{Grimmett1999}):
$$
E[\theta(t)] = 0 \mif p < \frac{1}{2}
$$
and
$$
E[\theta(t)] > 0 \mif p > \frac{1}{2},
$$
which is termed the \emph{percolation phenomenon}. In other words, there is a
\emph{critical density} above which a giant connected component appears
(\emph{super-critical phase}). Below this density, all connected components
have a finite size.

If the network is large but finite, its connectivity behavior is not much
different. Below the critical density, all connected components are relatively
small, and the largest of them may only contain a small fraction of the cars.
On the contrary, above the threshold, a large connected component forms, which
contains a large fraction of the cars (typically more than a half). Therefore,
a ``soft'' transition is expected, where the fraction of cars in the largest
cluster suddenly shifts from low values to values close to one.

We emphasize that these results are valid only if each and every road segment
is covered independently with the probability $p$. In practice, however, the
location of cars near intersections may influence the connectivity of the
adjacent segments. To cope with this dependence, we use two conditions, one
being necessary and the other sufficient for connectivity. This provides us and
upper and a lower bound on the connectivity.

The necessary condition is obtained by making the optimistic assumption that
there is at least one vehicle located at the center of each intersection. The
condition for the connectivity of a segment is thus that there is a sequence of
connected vehicles linking the two intersections. This condition only depends
on the location of the vehicles on the segment itself, and is thus independent
of any other segment. We denote by $p_u$ the probability that this condition is
fulfilled for a given segment. To compute $p_u$, we use Theorem~1 in
\cite{dousse02connectivity}, from which we obtain the formula:

$$
p_u = \left\{ \begin{array}{l}
1 \hspace{3.5cm} \mif 0 \leq L < r \\
\vspace{0.5ex}
\sum_{i=0}^{ \lfloor x/r \rfloor}
\frac{\left( -\lambda e^{-\lambda r} (x - ir) \right)^{i} }{i ! } \\
\;\;\; - e^{-\lambda r} \sum_{i=0}^{ \lfloor L/r \rfloor - 1}
\frac{\left( -\lambda e^{-\lambda r} (L - (i+1)r) \right)^{i} }{i ! } \\
\mbox{ } \hspace{3.8cm} \mif L \geq r \end{array} \right.
$$

The sufficient condition is obtained by assuming that each car is the center of
a disk of radius $r/2$ and requiring that the segment completely is covered by
disks (See Fig.~\ref{fig:balls}). As disks from consecutive cars must at least
touch each other, the distance between the centers is no more than $r$, and the
cars are connected. However, the ends of the segment might be covered by disks
from adjacent segments. The coverage thus depends also on the location of cars
in neighboring segments. To avoid this dependence, we simply strengthen the
condition by requiring that the segment is covered by disks centered on the
same segment. This leads to an independent condition, that is sufficient for
connectivity, and whose probability to be fulfilled $p_l$ can be computed using
the same theorem from \cite{dousse02connectivity}:

\begin{eqnarray*}
p_l &=& \sum_{i=0}^{ \lfloor L/r \rfloor+1} \frac{\left( -\lambda
e^{-\lambda r} (L - (i-1)r) \right)^{i} }{i ! } \\
& & - e^{-\lambda r} \sum_{i=0}^{ \lfloor L/r \rfloor} \frac{\left( -\lambda
e^{-\lambda r} (L - ir) \right)^{i} }{i ! }.
\end{eqnarray*}

\begin{figure}[htpb]
\psfrag{L}{\footnotesize $L$}
\psfrag{r/2}{\footnotesize $r/2$}
\includegraphics[width=\linewidth]{balls.eps}
\caption{Overlapping balls of radius $r/2$. If two adjacent segments are
completely covered with balls, the cars at the center of each ball are
necessarily connected.}
\label{fig:balls}
\end{figure}

Fig.~\ref{fig:connectivity} shows a comparison of the theoretical values of
$E[\theta(t)]$, using the necessary and sufficient conditions, and simulation
results. We see that despite the inaccuracy of the Poisson model in predicting
the detailed connectivity (isolated cars), the global connectivity matches the
model qualitatively. As expected, due to the finiteness of the simulated
network, the transition is much softer than in the theoretical model for
infinite networks. However, the threshold at which the fraction jumps is well
predicted by the model.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Percolation_probability.eps}
\caption{The two theoretical values and simulation of the fraction of cars in the largest cluster. The size of the simulation domain is $N=10$ and the scenario
is NL-A}
\label{fig:connectivity}
\end{figure}

\subsubsection{Simulation Analysis}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Biggest_cluster_function_car_density.eps}
\caption{Proportion of cars in the biggest vs. car density}
\label{fig:Biggest_cluster_function_car_density}
\end{figure}

As the theoretical analysis provided above hinges on the assumption
that vehicles are uniformly distributed in the network area, we
refrain from applying it for the settings with traffic lights. As
already seen through simulations, this is not the case for SL and GW,
especially more so for SL-R and GW-R. This is why we analyze the SL
and GW cases only through simulations, and plan to provide the
significantly more complex analysis in the journal version of the
paper. We ran simulations for both anti-diametric and random destinations
and will show the results for the anti-diametric destination scenarios only as we believe
they are enough to show the impact of the mobility regime on connectivity.

Fig.~\ref{fig:Biggest_cluster_function_car_density} shows the average
proportion of vehicles in the biggest cluster as a function of vehicle density
for SL and GW. We observe a major difference between SL-A and GW-A on the on
hand and NL-A (simple intersections) on the other hand. For NL-A,
$E[\theta(t)]$ increases with density ($\lambda$), and reaches 1 (i.e.,
(almost) all vehicles are connected. On the contrary, for the traffic-light
driven transportation, that is, for GW-A and SL-A,  $E[\theta(t)] < 0.35$. This
is explained if we observe the vehicle distribution and density for each
scenario. Fig.~\ref{fig:Car_density_Scenario1} shows that vehicle densities for
the scenario NL-A. We notice that, for vehicle density $\lambda < 60$
vehicles/Km, vehicles are equally distributed over the central and peripheral
roads. The network percolates when reaching the critical density: the cars form
one giant cluster.

%% #11# given the above statement, it would great here to have the SL-R and
%% GW-R

We consider the scenarios with traffic lights. We observe that the biggest
cluster size is bounded: $0.2E[n(t)]$ and $0.35E[n(t)] $ for the SL-A and GW-A
settings respectively. Interestingly, even though for SL-A higher density,
$\lambda$, is achieved (with increasing $f$ values) than that achieved for NL-A
(as shown in Sec.~\ref{sec:CarDensityfctCarFlow}), the SL-A largest cluster
size is lower that for NL-A. This can be explained by considering the traffic
dynamics: For SL, there exist basically two traffic phases: traffic lights
green, first, in the horizontal and then in the vertical direction. This
results in the formation of lengthy horizontal and vertical clusters, as those
shown in a snapshot of the network connectivity in
Fig.~\ref{fig:Biggest_cluster_flow400_Grid_5_400_tl}, that are disconnected
from each other. These ``parallel'' clusters of vehicles in motion never merge
into a large and eventually giant cluster in the range of scenarios we
investigate. On the other hand, for the GW setting, the central roads present a
very low density which is under the critical density. Thus, we remain in the
sub-critical phase and it explains the poor connectivity results: The network
does \emph{not} percolate and the proportion of cars in the biggest cluster is
logically the lower one among the three scenarios.


\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Biggest_cluster_flow400_Grid_5_400_tl.eps}
\caption{Example of a typical biggest cluster in the scenario SL-A. This snapshot corresponds to the release of the cars in
the vertical direction}
\label{fig:Biggest_cluster_flow400_Grid_5_400_tl}
\end{figure}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Isolated_cars_function_car_density.eps}
\caption{Proportion of isolated cars vs. car density}
\label{fig:Isolated_cars_function_car_density}
\end{figure}

Fig.~\ref{fig:Isolated_cars_function_car_density} shows the logarithm of the
average proportion of isolated cars, $\phi$, as a function of $\lambda$. A
straightforward observation is that increased density drives $\phi$ to zero.
Furthermore, we observe that $E[\phi(t)]$ is always lower for settings with
traffic lights (SL and GW), compared to no traffic lights (NL) settings. Again,
traffic lights hold vehicles at junctions, and those vehicles act as
``bridges'' for incident road segments. This is true even for low densities
(with no vehicles approaching from other directions): vehicles arriving at
traffic lights still stop. In contrast, this is not the case for simple
intersections and free-flow traffic.

\subsection{Critical Range}\label{sec:critical_range}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Critical_range_function_car_density.eps}
\caption{Critical range vs.cars density}
\label{fig:Critical_range_function_car_density}
\end{figure}

In this section, we investigate the minimum communication range needed to
obtain a large cluster (fully connected network), as a function of vehicle
density. The critical range is shown in
Fig.~\ref{fig:Critical_range_function_car_density} and it is, as one would
expected, a decreasing function of car density. We notice however that, for the
traffic lights scenario, the critical range surprisingly flattens when we
increase the car density from 110 to 150 vehicles/Km.\footnote{The critical
range is the mean over the duration of each of the randomly seeded simulation
runs. This implies that full connectivity is not guaranteed at all times, as
the maximum for example.} Recall that increasing the in-flow rate $f$ does not
lead to an ever-increasing density. For example, for NL, the maximum average
density achievable is approximately $110$ vehicles/Km, and the corresponding
curve in Fig.~\ref{fig:Critical_range_function_car_density} is truncated
accordingly.

%% To do
%% #17# We need a symbol for critical range

%% Too late...... :-(
%% #18# Once we have the look at the time-varying characteristics of connectivity,
%% we could perhaps argue that this is not a problem. We could promote to a paragraph here.

%% Too late.... :-(
%% #19# why not calculate the max critical range and the median and give side-by-side
%% those numbers?

On the other hand, when we consider the scenarios with traffic lights, we see
that even though the vehicle density increases the critical range does continue
to decrease. Rather, there is a minimum value of a critical range of
approximately 225 meters in the scenarios investigated here for SL and GW. The
reason for this and the faster convergence of the critical range for GW is
two-fold: (i) Central roads density remains lower and constant while that in
the peripheral roads continues to increase, and (ii) gaps in connectivity (if
the critical range were low) due to traffic lights. In other words, being
interested in the critical range, we should consider the sparser part of the
network, which is that of the central road segments. At the same time, an
increase in the density in central roads does not necessarily result in lower
critical range values: traffic lights essentially hold vehicles stopped, in
longer queues, while the higher range values are needed to connect those
stopped vehicles with the ones moving freely (not currently stopped by a
traffic light). The designer of vehicular communication protocols should take
into account this stop-and-go behavior, which is more pronounced in the SL, as
it causes inter-vehicle distance fluctuations and thus requires higher
communication ranges to ensure connectivity.

%% ????????????
%% #21# It would be interesting to comment on what is the case for SL-R. If the same,
%% then let's just say that the observations are good for both cases.

%% Too late ... :-(
%% #22# If we cannot create a separate subsection, we should interleave
%% in the discussion evidence on how things change dynamically over time.
%% I.e., is the size (proportion) of the largest cluster changing significantly
%% over time?

\subsection{VC Market Penetration} \label{sec:market_penetration}

In this section, we study the impact of Market penetration and background
traffic(non equipped cars) on connectivity based on simulations. We declare
each car that starts its trip to be equipped with probability $\rho$ and
measure the connectivity level. Simulations shows, as expected, that the
connectivity improves when increasing the market penetration: Increasing the
proportion of equipped cars increases the probability to have a neighbor which
is equipped and so improves the overall connectivity level. However, increasing
the background traffic does not only affect the proportion of equipped cars but
has an impact on the traffic.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_main_dest_no_tl,width=7cm}}
\caption{Scenario with no traffic lights and Anti-Diametric Destination}
\label{fig:flow400_main_dest_no_tl}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_main_dest_tl,width=7cm}}
\caption{Scenario with traffic lights and Anti-Diametric Destination}
\label{fig:flow400_main_dest_tl}\end{minipage}
\end{figure}

In Figs.~\ref{fig:flow400_main_dest_no_tl},~\ref{fig:flow400_main_dest_tl} we
consider the scenarios with anti-diametric trajectories : we observe that the
background effect has no significant effect on the connectivity level. Even
though the average proportion of isolated cars tends to increase or remain constant,
the average proportion of vehicles in the biggest cluster somewhat increases, but the
gain is not significant.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_dist_dest_no_tl,width=7cm}}
\caption{Scenario with no traffic lights and random Destination}
\label{fig:flow400_dist_dest_no_tl}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_dist_dest_tl,width=7cm}}
\caption{Scenario with synchronized traffic lights and random Destination}
\label{fig:flow400_dist_dest_tl}\end{minipage}
\end{figure}

Figs.~\ref{fig:flow400_dist_dest_no_tl} and
\ref{fig:flow400_dist_dest_tl} present results for the scenarios
with random destinations. We obtain unexpected and quite interesting
behavior of the average proportion of cars in the biggest cluster: this
quantity increases significantly when increasing the background
traffic and especially in the case where we have traffic lights at
intersections. How can the background traffic have an effect on the
connectivity and why do we have this phenomenon only for the case
when we have scenarios with distributed destinations? The key is the
effect of cars trips and so the distribution of destinations on the
traffic and cars distribution. Looking closely at the scenario with
random trajectories and no traffic lights (corresponding to the
Fig.~\ref{fig:flow400_dist_dest_no_tl}), the proportion of cars in
the biggest cluster decreases from ($\lambda = 24 \, Car/Km, \rho =
1, E[\theta(t)] = 0.4 $) to ($\lambda = 48 \, Car/Km, \rho = 0.51,
E[\theta(t)] = 0.34 $) and increased to ($\lambda = 163 \, Car/Km,
\rho = 0.15, E[\theta(t)] = 0.6 $). It is clear that the point
corresponding to ($\lambda = 48 \, Car/Km, \rho = 0.51, E[\theta(t)]
= 0.34 $) witnessed a kind of change, we plot the cars distribution
over time around this point: We divide the maps in small zones and
count the number of cars that went through in this zone over time.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_distribution_dist_dest_notl_flow500,width=7cm}}
\caption{Car distribution in the scenario NL-R for $\lambda=37 \, Car/Km$ . The z-axis corresponds to the mean number of cars at each time step.
We notice that the most dense spots are intersections.}
\label{fig:Car_distribution_dist_dest_notl_flow500}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_distribution_dist_dest_notl_flow600,width=7cm}}
\caption{Car distribution in the scenario 4 with NL-R for  $\lambda=65 \, Car/Km$. The z-axis corresponds to the mean number of cars at each time step. The central roads are really dense and cars are clustered}
\label{fig:Car_distribution_dist_dest_notl_flow600}\end{minipage}
\end{figure}

We see clearly that the spatial distribution of vehicles changes. In
Fig.~\ref{fig:Car_distribution_dist_dest_notl_flow500}, there is an
important car density at intersections while in
Fig.~\ref{fig:Car_distribution_dist_dest_notl_flow600}, the central
roads are congested too and show an important car density. This is
due to the fact that, in the distributed destinations scenarios, cars
have longer trips and are more likely to turn at intersections which incurs a delay in the
queues at intersections and leads to more dense central roads. We see
in Fig.~\ref{fig:Car_distribution_dist_dest_notl_flow600} that the
cars traffic is really forming a square in the central zone and
therefore, equipped cars are more likely to be in range of each other
to form clusters (while in the scenarios with main destinations, cars
are more likely to be at intersections and so out of the range of
each other). \newline We can conclude that as the background traffic affects
the mobility and distribution of equipped cars, it has an impact,
sometimes positive, on the connectivity level and more precisely on
the proportion of cars in the biggest cluster.


==> Connectivity_adhoc-2.tex <==
\section{Vehicle-to-Vehicle Connectivity} \label{Sec:EvalConneAd-hocNet}

This section presents our findings on vehicle-to-vehicle (V2V) connectivity,
based on analysis and extensive experiments with microscopic vehicle mobility
simulation. We consider urban grids of two-lane bidirectional roads, in the
shape of Fig.~\ref{fig:domain}, with the number of horizontal and vertical
perpendicular roads ranging from $N=5$ to $10$. The entry and destination
points for vehicles are at the edges of the grid, as explained in
Sec.~\ref{Sec:Models}.

At first, we seek to understand how vehicles are distributed across the road
grid, as a function of their entrance rate and for each of the three above
mentioned settings. Our findings, detailed in
Sec.~\ref{sec:CarDensityfctCarFlow}, show that the presence and mode of
operation of traffic has a significant impact on the density and spatial
distribution of vehicles.

The differing vehicle placement conditions, as a result of the differing rates
of entrance (and exit) from the simulated road grid, influence the overall
connectivity and most notably the proportion of vehicles in the largest
cluster. Clearly, the highest the proportion, the more likely it is to have any
piece of information disseminated to all vehicles in the cluster. But, as it
will be explained in Sec.~\ref{sec:cluster}, traffic lights significantly
influence the size of largest cluster.

%%%% CAPTION
\begin{figure*}[htpb]
\includegraphics[width=\linewidth]{Merged_density_plots_anti-diametric.eps}
\caption{ } \label{fig:d}
\end{figure*}

On a different dimension of our investigation, we consider the critical range,
that is the minimum communication range that enables all vehicles to belong to
a single cluster. Again, traffic lights heavily influence the value of the
critical range Sec.\ref{sec:critical_range}. We shift gears in
Sec.~\ref{sec:market_penetration}, where we are concerned with vehicular
networks comprising a fraction of the circulating vehicles. Now, the presence
of vehicles that are not equipped with radios essentially model the spatial
distribution of the equipped vehicles and thus the vehicular network
connectivity.

\begin{table}[htb]
\caption{Simulation parameters} \small\addtolength{\tabcolsep}{-5pt}
\begin{tabular}{|l|l|}
\hline
Simulation interval & [0,999s] \\
\hline
Number of lane & 2  \\
\hline
Grid dimension & 5, 10 \\
\hline
Traffic lights regimes & Synchronized, Green Wave\\
\hline
Road segment length $L$ [m] & 400 \\
\hline
$f$ (CarArrival/h/lane) & 100..1500\\
\hline
Types of destination & Anti-Diametric, Random\\
\hline \hline
Connectivity range $r$ [m] & 100\\
\hline
\end{tabular}
\end{table}

Throughout this section, we present results for the three types of road traffic
control, as described in Sec.~\ref{Sec:Models}, differentiated by the existence
and operation of traffic lights: ``\textbf{N}o Traffic \textbf{L}ights''
(\textbf{NL}), ``\textbf{S}ynchronized Traffic \textbf{L}ights'' (\textbf{SL}),
and ``\textbf{G}reen \textbf{W}ave'' (\textbf{GW}). We combine those settings
with different road destination selection settings, again described in
Sec.~\ref{Sec:Models}: ``\textbf{A}nti-diametric'' or ``\textbf{R}andom''
destination road end points. For example, SL-R signifies synchronized traffic
lights with random destinations. Note that the green wave regime can be
meaningful when cars can keep a constant speed. This is not the case for the
random destination model, where cars are more likely to turn at intersections,
decelerate or even stop before doing so, and thus cause significant velocity
fluctuations; this is why we do not investigate the GW-R case.

\subsection{Vehicle Density} \label{sec:CarDensityfctCarFlow}

As the simulator allows us to control the in-flow rate for each source (entry)
point, we utilize this as the independent parameter in our experiments.
Nonetheless, the resultant placement of vehicles is what is of real interest.
This is why we investigate how the entrance rate (for a given $N$ dimension of
the road network grid) relates to the average vehicle density. We note
nonetheless that vehicle density, and their spatial distribution more
generally, do not depend only on the flow of cars entering the network but also
on the mobility regime and cars trip.

%% Make them smaller
\begin{figure*}[htpb]
\includegraphics[width=\linewidth]{Merged_density_plots_random.eps}
\caption{} \label{fig:d}
\end{figure*}

%%% Finalize references to all figures
First, for all figures, we observe that there is a variation of the
distribution across the road network. We differentiate \emph{peripheral road
segments} as those $4N$ segments between the vehicle entry and exit points and
the first-encountered intersection. We term all the remaining road segments in
the grid as \emph{central road segments}.

We first look at the scenarios with anti-diametric destinations and observe
that, as the vehicle in-flow rate increases, the vehicle density increases in a
similar manner for peripheral and central road segments. But this only up to a
certain value of $f$, e.g., $f=800$ for Fig.~\ref{fig:Car_density_Scenario1},
after which the density in central roads increases very slowly and then does
not increase any further. While, the vehicle density in peripheral roads
continue to increase beyond that point, until it also reaches a plateau, for a
larger in-flow rate, e.g., $f=1000$ for Fig.~\ref{fig:Car_density_Scenario1}.
This phenomenon occurs consistently for all scenarios, but with different
transition $f$ values. Basically, central road segment $\lambda$ is lower for
the GW compared to SL and NL. At the same time, the differentiation between
peripheral and central segments occurs for lower $f$ values for GW, compared to
those for SL and NL.

These variations are due to the role of traffic lights. Looking, for example,
at Fig.~\ref{fig:Car_density_Scenario3}, the central road density flattens at
$f=500$vehicles/h/lane. This is so, because traffic lights at the first
intersection encountered by vehicles, that is, at the limit of each peripheral
road segment, control the in-flow to the central road segments. Essentially,
they act as a bottleneck. At this point, traffic jams start building up at the
peripheral roads, up to the point the density reaches, at
$f=800$vehicles/h/lane, a plateau: the jammed peripheral roads do not allow the
entrance of more vehicles. In contrast, without traffic lights, stop signs at
intersections start acting as a bottleneck only when the amount of traffic is
such that long queues build up at all sides of the intersection. This
essentially ``shifts'' the saturation point for $\lambda$ to occur for
$f>1000$. But it is interesting to see that for NL, the plateau occurs for
peripheral and central roads for that same $f$. Again, peripheral roads reach
higher densities, up to the point they get jammed.

On the other hand, for scenarios with random destination(s), we also observe
the saturation phenomenon and the differentiation between peripheral and
central road segments (Fig.~\ref{fig:Car_density_Scenario4}). However, central
roads get more congested than peripheral roads. This peculiarity stems from the
trip type: with random destinations vehicle routes are longer while vehicles
are more likely to turn at intersections to reach their destination. As a
consequence, cars stay longer in the (simulated) road network and especially in
central road segments.

\subsection{Vehicle Clustering}\label{sec:cluster}

We study the clustering of cars both from an analytical and simulation
approach. For the scenario where we have simple intersections, we show that
accurate predictions of the network connectivity can be made using percolation
theory. For the scenarios involving traffic lights, we study connectivity using
our microscopic simulator and show the main differences with the simple
intersections case.   

\subsubsection{Analytical study}

For low vehicle arrival rates, road traffic has little impact on the
distribution of the cars along the roads. In the stationary regime, we can
model it with a spatial Poisson process. Also, we neglect the width of the
streets and associate them with lines. We obtain a one-dimensional process
along each road whose intensity  $\lambda$ is related to the car arrival rate
through the formula
$$
\lambda = \frac{2f}{\bar{v}},
$$
where $\bar{v}$ denotes the average speed of the cars. The factor $2$ is due to the bi-directionality of traffic.

Given the Poisson assumption, one can compute an upper bound on the average
fraction $E[\phi(t)]$ of cars that are connected to no other car in the
stationary regime, that is, when the road network is at a state that the rate
of vehicles entering the road network is the same as the rate of vehicle
leaving it:
$$
E[\phi(t)] = \exp(-2\lambda \rho r).
$$

Fig.~\ref{fig:isolated} shows a comparison of the analytical curve
with simulation results. The Poisson approximation shows its
limitations: when the density of cars is not very low, the
intersections start to shape their spatial distribution. Cars that
are stopped at an intersection are typically not isolated, whereas
cars leaving an intersection are well spaced and likely to be
isolated.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Isolated_cars.eps}
\caption{Theoretical and simulated fraction of isolated cars in a scenario with no traffic lights and Anti-diametric destinations. The size of the simulation domain is $N=10$ and road segments are $L=400m$ long.}
\label{fig:isolated}
\end{figure}

To compute the fraction of vehicles (nodes) belonging to the largest connected
component, we start by looking at the probability $p$ that a road segment (i.e.
the portion of road located between two consecutive intersections) is covered
by a sequence of connected cars. We can then see the network as an edge
percolation model, where each road segment is \emph{covered} (or \emph{open})
with probability $p$.

Percolation theory allows us to address the case where the network has an
infinite size, namely when $N\rightarrow\infty$. Then it is well known that
(see for example \cite{Grimmett1999}):
$$
E[\theta(t)] = 0 \mif p < \frac{1}{2}
$$
and
$$
E[\theta(t)] > 0 \mif p > \frac{1}{2},
$$
which is termed the \emph{percolation phenomenon}. In other words, there is a
\emph{critical density} above which a giant connected component appears
(\emph{super-critical phase}). Below this density, all connected components
have a finite size.

If the network is large but finite, its connectivity behavior is not much
different. Below the critical density, all connected components are relatively
small, and the largest of them may only contain a small fraction of the cars.
On the contrary, above the threshold, a large connected component forms, which
contains a large fraction of the cars (typically more than a half). Therefore,
a ``soft'' transition is expected, where the fraction of cars in the largest
cluster suddenly shifts from low values to values close to one.

We emphasize that these results are valid only if each and every road segment
is covered independently with the probability $p$. In practice, however, the
location of cars near intersections may influence the connectivity of the
adjacent segments. To cope with this dependence, we use two conditions, one
being necessary and the other sufficient for connectivity. This provides us and
upper and a lower bound on the connectivity.

The necessary condition is obtained by making the optimistic assumption that
there is at least one vehicle located at the center of each intersection. The
condition for the connectivity of a segment is thus that there is a sequence of
connected vehicles linking the two intersections. This condition only depends
on the location of the vehicles on the segment itself, and is thus independent
of any other segment. We denote by $p_u$ the probability that this condition is
fulfilled for a given segment. To compute $p_u$, we use Theorem~1 in
\cite{dousse02connectivity}, from which we obtain the formula:

$$
p_u = \left\{ \begin{array}{l}
1 \hspace{3.5cm} \mif 0 \leq L < r \\
\vspace{0.5ex}
\sum_{i=0}^{ \lfloor x/r \rfloor}
\frac{\left( -\lambda e^{-\lambda r} (x - ir) \right)^{i} }{i ! } \\
\;\;\; - e^{-\lambda r} \sum_{i=0}^{ \lfloor L/r \rfloor - 1}
\frac{\left( -\lambda e^{-\lambda r} (L - (i+1)r) \right)^{i} }{i ! } \\
\mbox{ } \hspace{3.8cm} \mif L \geq r \end{array} \right.
$$

The sufficient condition is obtained by assuming that each car is the center of
a disk of radius $r/2$ and requiring that the segment completely is covered by
disks (See Fig.~\ref{fig:balls}). As disks from consecutive cars must at least
touch each other, the distance between the centers is no more than $r$, and the
cars are connected. However, the ends of the segment might be covered by disks
from adjacent segments. The coverage thus depends also on the location of cars
in neighboring segments. To avoid this dependence, we simply strengthen the
condition by requiring that the segment is covered by disks centered on the
same segment. This leads to an independent condition, that is sufficient for
connectivity, and whose probability to be fulfilled $p_l$ can be computed using
the same theorem from \cite{dousse02connectivity}:

\begin{eqnarray*}
p_l &=& \sum_{i=0}^{ \lfloor L/r \rfloor+1} \frac{\left( -\lambda
e^{-\lambda r} (L - (i-1)r) \right)^{i} }{i ! } \\
& & - e^{-\lambda r} \sum_{i=0}^{ \lfloor L/r \rfloor} \frac{\left( -\lambda
e^{-\lambda r} (L - ir) \right)^{i} }{i ! }.
\end{eqnarray*}

\begin{figure}[htpb]
\psfrag{L}{\footnotesize $L$}
\psfrag{r/2}{\footnotesize $r/2$}
\includegraphics[width=\linewidth]{balls.eps}
\caption{Overlapping balls of radius $r/2$. If two adjacent segments are
completely covered with balls, the cars at the center of each ball are
necessarily connected.}
\label{fig:balls}
\end{figure}

Fig.~\ref{fig:connectivity} shows a comparison of the theoretical values of
$E[\theta(t)]$, using the necessary and sufficient conditions, and simulation
results. We see that despite the inaccuracy of the Poisson model in predicting
the detailed connectivity (isolated cars), the global connectivity matches the
model qualitatively. As expected, due to the finiteness of the simulated
network, the transition is much softer than in the theoretical model for
infinite networks. However, the threshold at which the fraction jumps is well
predicted by the model.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Percolation_probability.eps}
\caption{The two theoretical values and simulation of the fraction of cars in the largest cluster. The size of the simulation domain is $N=10$ and the scenario
is NL-A}
\label{fig:connectivity}
\end{figure}

\subsubsection{Simulation Analysis}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Biggest_cluster_function_car_density.eps}
\caption{Proportion of cars in the biggest vs. car density}
\label{fig:Biggest_cluster_function_car_density}
\end{figure}

As the theoretical analysis provided above hinges on the assumption
that vehicles are uniformly distributed in the network area, we
refrain from applying it for the settings with traffic lights. As
already seen through simulations, this is not the case for SL and GW,
especially more so for SL-R and GW-R. This is why we analyze the SL
and GW cases only through simulations, and plan to provide the
significantly more complex analysis in the journal version of the
paper. We ran simulations for both anti-diametric and random destinations
and will show the results for the anti-diametric destination scenarios only as we believe
they are enough to show the impact of the mobility regime on connectivity.

Fig.~\ref{fig:Biggest_cluster_function_car_density} shows the average
proportion of vehicles in the biggest cluster as a function of vehicle density
for SL and GW. We observe a major difference between SL-A and GW-A on the on
hand and NL-A (simple intersections) on the other hand. For NL-A,
$E[\theta(t)]$ increases with density ($\lambda$), and reaches 1 (i.e.,
(almost) all vehicles are connected. On the contrary, for the traffic-light
driven transportation, that is, for GW-A and SL-A,  $E[\theta(t)] < 0.35$. This
is explained if we observe the vehicle distribution and density for each
scenario. Fig.~\ref{fig:Car_density_Scenario1} shows that vehicle densities for
the scenario NL-A. We notice that, for vehicle density $\lambda < 60$
vehicles/Km, vehicles are equally distributed over the central and peripheral
roads. The network percolates when reaching the critical density: the cars form
one giant cluster.

%% #11# given the above statement, it would great here to have the SL-R and
%% GW-R

We consider the scenarios with traffic lights. We observe that the biggest
cluster size is bounded: $0.2E[n(t)]$ and $0.35E[n(t)] $ for the SL-A and GW-A
settings respectively. Interestingly, even though for SL-A higher density,
$\lambda$, is achieved (with increasing $f$ values) than that achieved for NL-A
(as shown in Sec.~\ref{sec:CarDensityfctCarFlow}), the SL-A largest cluster
size is lower that for NL-A. This can be explained by considering the traffic
dynamics: For SL, there exist basically two traffic phases: traffic lights
green, first, in the horizontal and then in the vertical direction. This
results in the formation of lengthy horizontal and vertical clusters, as those
shown in a snapshot of the network connectivity in
Fig.~\ref{fig:Biggest_cluster_flow400_Grid_5_400_tl}, that are disconnected
from each other. These ``parallel'' clusters of vehicles in motion never merge
into a large and eventually giant cluster in the range of scenarios we
investigate. On the other hand, for the GW setting, the central roads present a
very low density which is under the critical density. Thus, we remain in the
sub-critical phase and it explains the poor connectivity results: The network
does \emph{not} percolate and the proportion of cars in the biggest cluster is
logically the lower one among the three scenarios.


\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Biggest_cluster_flow400_Grid_5_400_tl.eps}
\caption{Example of a typical biggest cluster in the scenario SL-A. This snapshot corresponds to the release of the cars in
the vertical direction}
\label{fig:Biggest_cluster_flow400_Grid_5_400_tl}
\end{figure}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Isolated_cars_function_car_density.eps}
\caption{Proportion of isolated cars vs. car density}
\label{fig:Isolated_cars_function_car_density}
\end{figure}

Fig.~\ref{fig:Isolated_cars_function_car_density} shows the logarithm of the
average proportion of isolated cars, $\phi$, as a function of $\lambda$. A
straightforward observation is that increased density drives $\phi$ to zero.
Furthermore, we observe that $E[\phi(t)]$ is always lower for settings with
traffic lights (SL and GW), compared to no traffic lights (NL) settings. Again,
traffic lights hold vehicles at junctions, and those vehicles act as
``bridges'' for incident road segments. This is true even for low densities
(with no vehicles approaching from other directions): vehicles arriving at
traffic lights still stop. In contrast, this is not the case for simple
intersections and free-flow traffic.

\subsection{Critical Range}\label{sec:critical_range}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Critical_range_function_car_density.eps}
\caption{Critical range vs.cars density}
\label{fig:Critical_range_function_car_density}
\end{figure}

In this section, we investigate the minimum communication range needed to
obtain a large cluster (fully connected network), as a function of vehicle
density. The critical range is shown in
Fig.~\ref{fig:Critical_range_function_car_density} and it is, as one would
expected, a decreasing function of car density. We notice however that, for the
traffic lights scenario, the critical range surprisingly flattens when we
increase the car density from 110 to 150 vehicles/Km.\footnote{The critical
range is the mean over the duration of each of the randomly seeded simulation
runs. This implies that full connectivity is not guaranteed at all times, as
the maximum for example.} Recall that increasing the in-flow rate $f$ does not
lead to an ever-increasing density. For example, for NL, the maximum average
density achievable is approximately $110$ vehicles/Km, and the corresponding
curve in Fig.~\ref{fig:Critical_range_function_car_density} is truncated
accordingly.

%% To do
%% #17# We need a symbol for critical range

%% Too late...... :-(
%% #18# Once we have the look at the time-varying characteristics of connectivity,
%% we could perhaps argue that this is not a problem. We could promote to a paragraph here.

%% Too late.... :-(
%% #19# why not calculate the max critical range and the median and give side-by-side
%% those numbers?

On the other hand, when we consider the scenarios with traffic lights, we see
that even though the vehicle density increases the critical range does continue
to decrease. Rather, there is a minimum value of a critical range of
approximately 225 meters in the scenarios investigated here for SL and GW. The
reason for this and the faster convergence of the critical range for GW is
two-fold: (i) Central roads density remains lower and constant while that in
the peripheral roads continues to increase, and (ii) gaps in connectivity (if
the critical range were low) due to traffic lights. In other words, being
interested in the critical range, we should consider the sparser part of the
network, which is that of the central road segments. At the same time, an
increase in the density in central roads does not necessarily result in lower
critical range values: traffic lights essentially hold vehicles stopped, in
longer queues, while the higher range values are needed to connect those
stopped vehicles with the ones moving freely (not currently stopped by a
traffic light). The designer of vehicular communication protocols should take
into account this stop-and-go behavior, which is more pronounced in the SL, as
it causes inter-vehicle distance fluctuations and thus requires higher
communication ranges to ensure connectivity.

%% ????????????
%% #21# It would be interesting to comment on what is the case for SL-R. If the same,
%% then let's just say that the observations are good for both cases.

%% Too late ... :-(
%% #22# If we cannot create a separate subsection, we should interleave
%% in the discussion evidence on how things change dynamically over time.
%% I.e., is the size (proportion) of the largest cluster changing significantly
%% over time?

\subsection{VC Market Penetration} \label{sec:market_penetration}

In this section, we study the impact of Market penetration and background
traffic(non equipped cars) on connectivity based on simulations. We declare
each car that starts its trip to be equipped with probability $\rho$ and
measure the connectivity level. Simulations shows, as expected, that the
connectivity improves when increasing the market penetration: Increasing the
proportion of equipped cars increases the probability to have a neighbor which
is equipped and so improves the overall connectivity level. However, increasing
the background traffic does not only affect the proportion of equipped cars but
has an impact on the traffic.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_main_dest_no_tl,width=7cm}}
\caption{Scenario with no traffic lights and Anti-Diametric Destination}
\label{fig:flow400_main_dest_no_tl}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_main_dest_tl,width=7cm}}
\caption{Scenario with traffic lights and Anti-Diametric Destination}
\label{fig:flow400_main_dest_tl}\end{minipage}
\end{figure}

In Figs.~\ref{fig:flow400_main_dest_no_tl},~\ref{fig:flow400_main_dest_tl} we
consider the scenarios with anti-diametric trajectories : we observe that the
background effect has no significant effect on the connectivity level. Even
though the average proportion of isolated cars tends to increase or remain constant,
the average proportion of vehicles in the biggest cluster somewhat increases, but the
gain is not significant.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_dist_dest_no_tl,width=7cm}}
\caption{Scenario with no traffic lights and random Destination}
\label{fig:flow400_dist_dest_no_tl}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_dist_dest_tl,width=7cm}}
\caption{Scenario with synchronized traffic lights and random Destination}
\label{fig:flow400_dist_dest_tl}\end{minipage}
\end{figure}

Figs.~\ref{fig:flow400_dist_dest_no_tl} and
\ref{fig:flow400_dist_dest_tl} present results for the scenarios
with random destinations. We obtain unexpected and quite interesting
behavior of the average proportion of cars in the biggest cluster: this
quantity increases significantly when increasing the background
traffic and especially in the case where we have traffic lights at
intersections. How can the background traffic have an effect on the
connectivity and why do we have this phenomenon only for the case
when we have scenarios with distributed destinations? The key is the
effect of cars trips and so the distribution of destinations on the
traffic and cars distribution. Looking closely at the scenario with
random trajectories and no traffic lights (corresponding to the
Fig.~\ref{fig:flow400_dist_dest_no_tl}), the proportion of cars in
the biggest cluster decreases from ($\lambda = 24 \, Car/Km, \rho =
1, E[\theta(t)] = 0.4 $) to ($\lambda = 48 \, Car/Km, \rho = 0.51,
E[\theta(t)] = 0.34 $) and increased to ($\lambda = 163 \, Car/Km,
\rho = 0.15, E[\theta(t)] = 0.6 $). It is clear that the point
corresponding to ($\lambda = 48 \, Car/Km, \rho = 0.51, E[\theta(t)]
= 0.34 $) witnessed a kind of change, we plot the cars distribution
over time around this point: We divide the maps in small zones and
count the number of cars that went through in this zone over time.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_distribution_dist_dest_notl_flow500,width=7cm}}
\caption{Car distribution in the scenario NL-R for $\lambda=37 \, Car/Km$ . The z-axis corresponds to the mean number of cars at each time step.
We notice that the most dense spots are intersections.}
\label{fig:Car_distribution_dist_dest_notl_flow500}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_distribution_dist_dest_notl_flow600,width=7cm}}
\caption{Car distribution in the scenario 4 with NL-R for  $\lambda=65 \, Car/Km$. The z-axis corresponds to the mean number of cars at each time step. The central roads are really dense and cars are clustered}
\label{fig:Car_distribution_dist_dest_notl_flow600}\end{minipage}
\end{figure}

We see clearly that the spatial distribution of vehicles changes. In
Fig.~\ref{fig:Car_distribution_dist_dest_notl_flow500}, there is an
important car density at intersections while in
Fig.~\ref{fig:Car_distribution_dist_dest_notl_flow600}, the central
roads are congested too and show an important car density. This is
due to the fact that, in the distributed destinations scenarios, cars
have longer trips and are more likely to turn at intersections which incurs a delay in the
queues at intersections and leads to more dense central roads. We see
in Fig.~\ref{fig:Car_distribution_dist_dest_notl_flow600} that the
cars traffic is really forming a square in the central zone and
therefore, equipped cars are more likely to be in range of each other
to form clusters (while in the scenarios with main destinations, cars
are more likely to be at intersections and so out of the range of
each other). \newline We can conclude that as the background traffic affects
the mobility and distribution of equipped cars, it has an impact,
sometimes positive, on the connectivity level and more precisely on
the proportion of cars in the biggest cluster.


==> Connectivity_adhoc-pp.tex <==
\section{Vehicle-to-Vehicle Connectivity} \label{Sec:EvalConneAd-hocNet}

This section presents our findings on vehicle-to-vehicle (V2V) connectivity,
based on analysis and extensive experiments with microscopic vehicle mobility
simulation. We consider urban grids of two-lane bidirectional roads, in the
shape of Fig.~\ref{fig:domain}, with the number of horizontal and vertical
perpendicular roads ranging from $N=5$ to $10$. The entry and destination
points for vehicles are at the edges of the grid, as explained in
Sec.~\ref{Sec:Models}.

At first, we seek to understand how vehicles are distributed across the road
grid, as a function of their entrance rate and for each of the three above
mentioned settings. Our findings, detailed in
Sec.~\ref{sec:CarDensityfctCarFlow}, show that the presence and mode of
operation of traffic has a significant impact on the density and spatial
distribution of vehicles.

The differing vehicle placement conditions, as a result of the differing rates
of entrance (and exit) from the simulated road grid, influence the overall
connectivity and most notably the proportion of vehicles in the largest
cluster. Clearly, the highest the proportion, the more likely it is to have any
piece of information disseminated to all vehicles in the cluster. But, as it
will be explained in Sec.~\ref{sec:cluster}, traffic lights significantly
influence the size of largest cluster.

On a different dimension of our investigation, we consider the critical range,
that is the minimum communication range that enables all vehicles to belong to
a single cluster. Again, traffic lights heavily influence the value of the
critical range Sec.\ref{sec:critical_range}. We shift gears in
Sec.~\ref{sec:market_penetration}, where we are concerned with vehicular
networks comprising a fraction of the circulating vehicles. Now, the presence
of vehicles that are not equipped with radios essentially model the spatial
distribution of the equipped vehicles and thus the vehicular network
connectivity.

Throughout this section, we present results for the three types of road traffic
control, as described in Sec.~\ref{Sec:Models}, differentiated by the existence
and operation of traffic lights: ``\textbf{N}o Traffic \textbf{L}ights''
(\textbf{NL}), ``\textbf{S}ynchronized Traffic \textbf{L}ights'' (\textbf{SL}),
and ``\textbf{G}reen \textbf{W}ave'' (\textbf{GW}). We combine those settings
with different road destination selection settings, again described in
Sec.~\ref{Sec:Models}: ``\textbf{A}nti-diametric'' or ``\textbf{R}andom''
destination road end points. For example, SL-R signifies synchronized traffic
lights with random destinations.

\begin{table}[htb]
\caption{Simulation parameters}
\small\addtolength{\tabcolsep}{-5pt}
\begin{tabular}{|l|l|}
\hline
Simulation interval & [0,999s] \\
\hline
Number of lane & 2  \\
\hline
Grid dimension & 5, 10, 20 \\
\hline
Traffic lights regimes & Synchronized, Green Wave\\
\hline
Road segment length $L$ [m] & 400 \\
\hline
$f$ (CarArrival/h/lane) & 100..1500\\
\hline
Types of destination & Anti-Diametric, Random\\
\hline
\hline
Connectivity range $r$ [m] & 100\\
\hline
\end{tabular}
\end{table}


\subsection{Vehicle Density} \label{sec:CarDensityfctCarFlow}

As the simulator allows us to control the in-flow rate for each source (entry)
point, we utilize this as the independent parameter in our experiments.
Nonetheless, the resultant placement of vehicles is what is of real interest.
This is why we investigate how the entrance rate (for a given $N$ dimension of
the road network grid) relates to the average vehicle density. We note
nonetheless that vehicle density, and their spatial distribution more
generally, do not depend only on the flow of cars entering the network but also
on the mobility regime, as shown in
Figs.~\ref{fig:Car_density_Scenario1,fig:Car_density_Scenario2,fig:Car_density_Scenario3}.
%% TO BE CHANGED INTO ONE FIGURE

First, for all figures, we observe that there is a variation of the
distribution across the road network. We differentiate \emph{peripheral road
segments} as those $4N$ segments between the vehicle entry and exit points and
the first-encountered intersection. We term all the remaining road segments in
the grid as \emph{central road segments}. As the vehicle in-flow rate
increases, the vehicle density increases in a similar manner for peripheral and
central road segments. But this only up to a certain value of $f$, e.g.,
$f=800$ for Fig.~\ref{fig:Car_density_Scenario1}, after which the density in
central roads increases very slowly and then does not increase any further.
While, the vehicle density in peripheral roads continue to increase beyond that
point, until it also reaches a plateau, for a lager in-flow rate, e.g.,
$f=1000$ for Fig.~\ref{fig:Car_density_Scenario1}. This phenomenon occurs
consistently for all scenarios, but with different transition $f$ values.
Basically, central road segment $\lambda$ is lower for the GW compared to SL
and NL. %%% WHY? THIS IS NOT CLEAR!

At the same time, the differentiation between peripheral and central segments
occurs for lower $f$ values for GW, compared to SL and NL.


%% Discussion on results with Random destinations
For example, the traffic lights have an important impact on the cars
distribution and density over time. First, we notice in Figure
~\ref{fig:Car_density_Scenario3} that for the GW scenario, the cars
density flattens in the central zone flattens starting from flow equal to 500
Car Arrival/hour/lane which is due to the regulation of the traffic by the
traffic lights: At each phase, the traffic lights release the same number of
cars in the network. Logically, we notice the same phenomenon in the synchronized
traffic lights scenario, starting from a flow equal to 800 Vehicles/hour/lane,
the cars density in the central zone remains constant. Notice that in those
cases, traffic jams form at the entering points of the map where the density of
cars will be more important.\newline Concerning the scenario NL, we notice the flattening phenomena, for a flow of 1500
Vehicles/hour/lane, but it corresponds to the saturated regime where the
network becomes almost static.

\begin{figure}[htpb]
%\begin{minipage}{0.5\textwidth}
 \centerline{\epsfig{figure=Car_density_Scenario1,width=\linewidth}}
\caption{Car density vs. Car flow in the scenario NL-A}
\label{fig:Car_density_Scenario1}%\end{minipage}
%\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_density_scenario2,width=\linewidth}}
\caption{Car density vs. Car flow in the scenario SL-A}
\label{fig:Car_density_Scenario2}%\end{minipage}
\end{figure}
\begin{figure}[htpb]
%\begin{minipage}{0.5\linewidth}
\centerline{\epsfig{figure=Car_density_scenario3,width=\linewidth}}
\caption{Car density vs. Car flow in the scenario GW-A}
\label{fig:Car_density_Scenario3}%\end{minipage}
\end{figure}


\subsection{Vehicle Clustering}\label{sec:cluster}

We study the clustering of cars both from an analytical and simulation approach. For the simple intersections scenario, where the car density is low, we show that accurate predictions can be made of the connectivity of the network using percolation theory. For more complex cases, in particular those involving traffic lights and congestion, we study connectivity using our simulator and show the main differences with the simple case.

\subsubsection{Analytical study}

When the car arrival rate is low enough, road traffic has little impact on the distribution of the cars along the roads.
In the stationary regime, we can model it with a spatial Poisson process. Also, we neglect the width of the streets and associate them with lines. We obtain a one-dimensional process along each road whose intensity is denoted by $\lambda$.
Given the Poisson assumption, one can compute an upper bound on the average fraction $E[\phi(t)]$ of cars that are connected to no other car in the stationary regime:
$$
E[\phi(t)] = \exp(-2\lambda \rho r).
$$
Figure \ref{fig:isolated} shows a comparison of the analytical curve with simulation results. The Poisson approximation shows its limitations: when the density of cars is not very low, the intersections start to shape their spatial distribution. Cars that are stopped at an intersection are typically not isolated, whereas cars leaving an intersection are well spaced and likely to be isolated.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Isolated_cars.eps}
\caption{Theoretical and simulated fraction of isolated cars in a scenario NL-A. The size of the simulation domain is $N=10$ and road segment are $L=400m$ long.}
\label{fig:isolated}
\end{figure}

To compute the fraction of cars belonging to the largest connected component, we  start by looking at the probability
$p$ that a road segment (i.e. the portion of road located between two consecutive intersections) is covered by a sequence of connected cars. We can then see the network as an edge percolation model, where each road segment is \emph{covered} (or \emph{open}) with probability $p$.

Percolation theory allows to address the case where the network has an infinite size, namely when $N\rightarrow\infty$. Then it is well known that (see e.g. \cite{Grimmett1999})
$$
E[\theta(t)] = 0 \mif p < \frac{1}{2}
$$
and
$$
E[\theta(t)] > 0 \mif p > \frac{1}{2},
$$
which is called the \emph{percolation phenomenon}.
In other words, there is a critical density above which a giant connected component appears (\emph{super-critical phase}). Below this density, all connected components have a finite size.

If the network is large but finite, its connectivity behavior is not much different. Below the critical density, all connected components are relatively small, and the largest of them may only contain a small fraction of the cars. On the contrary, above the threshold, a large connected component forms, which contains a large fraction of the cars (typically more than a half). Therefore, a "soft" transition is expected, where the fraction of cars in the largest cluster suddenly shifts from low values to values close to one.

However, these results are only valid if road segments are declared covered independently form each other with the same probability $p$. In practice, the location of cars near intersections may influence the connectivity of the adjacent segments. To cope with this dependence, we use two conditions, one being necessary and the other sufficient for connectivity. This provides us and upper and a lower bound on the connectivity.

The necessary condition is obtained by making the optimistic assumption that there is at least one vehicle located at the center of each intersection. The condition for the connectivity of a segment is thus that there is a sequence of connected vehicles linking the two intersections. This condition only depends on the location of the vehicles on the segment itself, and is thus independent of any other segment. We denote by $p_u$ the probability that this condition is fulfilled for a given segment.

To compute $p_u$, we use Theorem~1 in \cite{dousse02connectivity}, from which we obtain the formula:
$$
p_u = \left\{ \begin{array}{l}
1 \hspace{3.5cm} \mif 0 \leq L < r \\
\vspace{0.5ex}
\sum_{i=0}^{ \lfloor x/r \rfloor}
\frac{\left( -\lambda e^{-\lambda r} (x - ir) \right)^{i} }{i ! } \\
\;\;\; - e^{-\lambda r} \sum_{i=0}^{ \lfloor L/r \rfloor - 1}
\frac{\left( -\lambda e^{-\lambda r} (L - (i+1)r) \right)^{i} }{i ! } \\
\mbox{ } \hspace{3.8cm} \mif L \geq r \end{array} \right.
$$

The sufficient condition is obtained by assuming that each car is the center of a disk of radius $r/2$ and requiring that the segment completely is covered by disks (see Figure~\ref{fig:balls}). As disks from consecutive cars must at least touch each other, the distance between the centers is no more than $r$, and the cars are connected.
However, the ends of the segment might be covered by disks from adjacent segments. The coverage thus depends also on the location of cars in neighboring segments. To avoid this dependence, we simply strengthen the condition by requiring that the segment is covered by disks centered on the same segment. This leads to an independent condition, that is sufficient for connectivity, and whose probability to be fulfilled $p_l$ can be computed using the same theorem from \cite{dousse02connectivity}:
\begin{eqnarray*}
p_l &=& \sum_{i=0}^{ \lfloor L/r \rfloor+1} \frac{\left( -\lambda
e^{-\lambda r} (L - (i-1)r) \right)^{i} }{i ! } \\
& & - e^{-\lambda r} \sum_{i=0}^{ \lfloor L/r \rfloor} \frac{\left( -\lambda
e^{-\lambda r} (L - ir) \right)^{i} }{i ! }.
\end{eqnarray*}

\begin{figure}[htpb]
\psfrag{L}{\footnotesize $L$}
\psfrag{r/2}{\footnotesize $r/2$}
\includegraphics[width=\linewidth]{balls.eps}
\caption{Overlapping balls of radius $r/2$. If two adjacent segments are completely covered with balls, the cars at the center of each ball are necessarily connected.}
\label{fig:balls}
\end{figure}

Figure \ref{fig:connectivity} shows a comparison of the theoretical values of $E[\theta(t)]$, using the necessary and sufficient conditions, and simulation results. We see that despite the inaccuracy of the Poisson model in predicting the detailed connectivity (isolated cars), the global connectivity qualitatively matches the model. As expected, due to the finiteness of the simulated network, the transition is much softer than in the theoretical model for infinite networks. However, the threshold at which the fraction jumps is well predicted by the model.
% *********************** COMMENT ON THE NEW PLOT *********************

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Percolation_probability.eps}
\caption{The two theoretical values and simulation of the fraction of cars in the largest cluster.}
\label{fig:connectivity}
\end{figure}

\subsubsection{Simulation experiments}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Biggest_cluster_function_car_density.eps}
\caption{Proportion of cars in the biggest vs. car density}
\label{fig:Biggest_cluster_function_car_density}
\end{figure}

Figure ~\ref{fig:Biggest_cluster_function_car_density} shows the
average proportion of cars belonging to the biggest cluster as a function of
the car density. The different curves correspond to different
simulation scenarios.\newline We observe a major difference between
the scenarios with traffic lights and the one with simple
intersections. In fact, the average proportion of cars belonging to the
biggest cluster increases with the car flow to reach 1 in the 
scenarios with simple intersections while it is upper bounded by $0.35E[n(t)]$ in the
traffic lights scenarios. We can explain the behavior of the biggest
cluster by observing the cars distribution and density for each
scenario. The Figure ~\ref{fig:Car_density_Scenario1} shows the car
densities at different roads for the scenario NL-A. We notice that,
for the values of flow lower than $800$ $cars/h/lane$(corresponding
to a car density lower than $60 car/Km$), the cars are equally
distributed over the roads and the network percolates: the cars form
one big cluster.

If we consider the scenarios with traffic lights and compare SL-A to the GW-A,
We notice that we obtain a bounded biggest cluster($0.35E[n(t)]$ and $0.2E[n(t)] $
for respectively SL-A and GW-A) even if the car
densities and distribution present very different characteristics. We
notice in Fig.~\ref{fig:Car_density_Scenario2} that, even if the
scenario SL presents also a quite fair car distribution and a
higher car density than the  scenario NL, the average size of the biggest
cluster is lower and upper bounded by $0.35E[n(t)]$. To explain this
phenomenon, we need to focus on the dynamic of the traffic: the
synchronized traffic lights present two distinct traffic phases
corresponding respectively to the moments where the traffic lights
are green for the horizontal and vertical direction. For both phases,
there is formation of linear and parallel clusters of cars in motion.
Those clusters, which are shown in
Fig.~\ref{fig:Biggest_cluster_flow400_Grid_5_400_tl}, never merge
into one big cluster as they are separated by a non connected
orthogonal road.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Biggest_cluster_flow400_Grid_5_400_tl.eps}
\caption{Example of a typical biggest cluster in the scenario SL-A. This snapshot corresponds to the release of the cars in 
the vertical direction}
\label{fig:Biggest_cluster_flow400_Grid_5_400_tl}
\end{figure}

As shown in Fig.~\ref{fig:Car_density_Scenario3}, Scenario GW differs
from Scenarios NL and SL: the central roads present a very low density
which is under the critical density. We remain in the sub-critical
phase and it explains the poor connectivity results: The network does
not percolate and the proportion of cars in the biggest cluster is
logically the lower one among the three scenarios. Traffic jams
occurs at the feeding points of the network(there is more cars than
the traffic light can handle) and the peripheral roads become really
congested which leads to the formation of small(less than $0.2E[n(t)]$)
clusters at the boundaries of the grid plan map. Those clusters
remain isolated and never merge into one spanning cluster.

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Isolated_cars_function_car_density.eps}
\caption{Proportion of isolated cars vs. car density}
\label{fig:Isolated_cars_function_car_density}
\end{figure}

Fig.~\ref{fig:Isolated_cars_function_car_density} shows the
average proportion of isolated cars as a function of the cars density. The
plot confirms the intuition that the proportion of isolated cars
tends to zero as we increase the traffic flow. The proportion of
isolated cars is always less in the traffic lights scenarios. This
can be explained by the role of meeting point played by the traffic
lights and the higher car densities for the same flow values. For low
car densities, a car has to stop in the traffic light even if there
is no car coming in the other directions. This is not the case when
we have simple intersections and free-flow traffic where cars meet
less often than in the traffic lights case.\newline If we consider
only the traffic lights scenarios, we notice that the proportion of
isolated cars is more important when we adopt the green-wave
strategy. This difference is more emphasized for low values of flow
and can be explained by the fact that the "green wave" gives more
improvement to the traffic flow in comparison with the synchronized
strategy at low values of flow. As showed in Fig.
~\ref{fig:Car_density_Scenario3}, central roads are less congested
when adopting the "green wave" strategy and there is less chance for
a car arriving to have another car in range.

\subsection{Critical Range}\label{sec:critical_range}

\begin{figure}[htpb]
\includegraphics[width=\linewidth]{Critical_range_function_car_density.eps}
\caption{Critical range vs.cars density}
\label{fig:Critical_range_function_car_density}
\end{figure}

The plot shows the critical range as a function of cars density. For
each flow, we took the mean of the critical range over the
simulation. The mean does not guarantee full connectivity for each
time step but is more relevant to us. We could consider the maximum
of the critical ranges over the simulation (the range that guarantee
full connectivity over the hole simulation) but it would reflect the
most isolated cars position instead of the range needed to ensure a
full connectivity while allowing temporary and isolated network
disconnections.\newline The critical range is, as expected, a
decreasing function of car density. We notice however that, for the traffic lights scenario,
the critical range surprisingly flattens when we increase the car
density from 110 to 150 car/Km (which corresponds to a flow increase from
800 to 1500 cars/h/lane ). This confirms what we saw before and the
fact that above a given density the connectivity remains flat. This
phenomenon is due to the gap between the cars that have just left the
traffic light and the ones still waiting for their turn and, even if
we increase the car density, this distance remains logically the
same.\newline So when designing VANETs, we have to take into account the
stop and go behavior (which is more important in the synchronized traffic lights scenario)
that causes the distance fluctuation and can lead to disconnections and important path breakages for example.

\subsection{VC Market Penetration} \label{sec:market_penetration}

As the market penetration will be probably low at the implementation
of such a network, it is interesting to study its effect on
connectivity. Furthermore, as the traffic will be composed by
equipped and non equipped cars, what will be the effect of the
background traffic (non equipped cars)on connectivity.\newline To
study the impact of market penetration, we declare each car that
starts its trip is declared to be equipped with probability $\rho$
: It is a Bernoulli process with probability of success $\rho$.

\subsubsection{Effect of Background Vehicular Traffic} \label{sec:EffectBackTraffic}

In this section, we want to study the impact of the background
traffic i.e. the effect of unequipped cars on connectivity. If we
keep the same number of equipped cars and increase the number of
unequipped cars. What impact will we have on connectivity?

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_main_dest_no_tl,width=7cm}}
\caption{Scenario with no traffic lights and Anti-Diametric Destination}
\label{fig:flow400_main_dest_no_tl}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_main_dest_tl,width=7cm}}
\caption{Scenario with traffic lights and Anti-Diametric Destination}
\label{fig:flow400_main_dest_tl}\end{minipage}
\end{figure}
In
Figs.~\ref{fig:flow400_main_dest_no_tl},~\ref{fig:flow400_main_dest_tl}
we consider the scenarios with Anti-Diamteric destinations : we observe that the background effect
has no significant effect on the connectivity level. Even though the
proportion of isolated cars tends to increase or remain constant, the
proportion of vehicles in the biggest cluster somewhat increases, but
the gain is not significant.

\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_dist_dest_no_tl,width=7cm}}
\caption{Scenario with no traffic lights and random Destination}
\label{fig:flow400_dist_dest_no_tl}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=flow400_dist_dest_tl,width=7cm}}
\caption{Scenario with synchronized traffic lights and random Destination}
\label{fig:flow400_dist_dest_tl}\end{minipage}
\end{figure}

Figs.~\ref{fig:flow400_dist_dest_no_tl}  and
~\ref{fig:flow400_dist_dest_tl} present results for the scenarios  with random
destinations. We obtain unexpected and quite interesting behavior of
the proportion of cars in the biggest cluster: this quantity
increases significantly when increasing the background traffic and
especially in the case where we have traffic lights at intersections.
How can the background traffic have an effect on the connectivity and
why do we have this phenomenon only for the case when we have
scenarios with random destinations? The key is the effect of
cars trips and so the distribution of destinations on the traffic and
cars distribution. Looking closely at  the scenario with random destinations
 and no traffic lights (corresponding to
the Fig. ~\ref{fig:flow400_dist_dest_no_tl}), the proportion of cars in the biggest
cluster decreases from ($\lambda = 24 \, Car/Km, \rho = 1, E[\theta(t)] = 0.4 $) to
($\lambda = 48 \, Car/Km, \rho = 0.51, E[\theta(t)] = 0.34 $) and
increased to ($\lambda = 163 \, Car/Km, \rho = 15, E[\theta(t)] = 0.6 $). It is clear that the point
corresponding to ($\lambda = 48 \, Car/Km, \rho = 0.51, E[\theta(t)] = 0.34 $) witnessed a
kind of change, we plot the cars distribution
over time around this point: We divide the maps in small zones and
count the number of cars that went through in this zone over
time.\newline
\begin{figure}[htpb]
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_distribution_dist_dest_notl_flow500,width=7cm}}
\caption{Car distribution in the scenario NL-R for $\lambda=37 \, Car/Km$ . The z-axis corresponds to the mean number of cars at each time step. 
We notice that the most dense spots are intersections.}
\label{fig:Car_distribution_dist_dest_notl_flow500}\end{minipage}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfig{figure=Car_distribution_dist_dest_notl_flow600,width=7cm}}
\caption{Car distribution in the scenario 4 with NL-R for  $\lambda=65 \, Car/Km$. The z-axis corresponds to the mean number of cars at each time step. The central roads are really dense and cars are clustered}
\label{fig:Car_distribution_dist_dest_notl_flow600}\end{minipage}
\end{figure}
We see clearly that the distribution of cars has changed. In Figure ~\ref{fig:Car_distribution_dist_dest_notl_flow500}, there is an important car density at intersections while in Figure ~\ref{fig:Car_distribution_dist_dest_notl_flow600}, the central roads are congested too and show an important car density. This is due to the fact that, in the random destinations scenarios, cars are more likely to turn at intersections and have longer trips which incurs a delay in the queues at intersections and a more important mean travel time. We see in Figure ~\ref{fig:Car_distribution_dist_dest_notl_flow600} that the cars traffic is really forming a square in the central zone and therefore, equipped cars are more likely to be in range of each other to form clusters (while in the scenarios with anti-diamteric destinations, cars are more likely to be at intersections and so out of the range of each other). \newline
We can conclude that as the background affects the mobility and distribution of equipped cars, it has an impact, sometimes positive, on the connectivity level and more precisely on the proportion of cars in the biggest cluster.


==> sumo.tex <==
We use SUMO~\cite{sumo}, as microscopic, continuous-space and discrete-time
traffic simulator to model realistic vehicle behavior. SUMO simulates the movement 
of every single vehicle implementing \emph{vehicle following model}  for 
vehicle movement (The driver behavior depends on the behavior and the speed 
of the car in front of him) and the \emph{dynamic user assignment} to find out the route to take. 
Driver decides in real time which route to take and his choice is not only
motivated by the route length but also by the mean speed within it. We obtain a realistic
behavior where drivers can change their route if it gets congested and take a
longer but less congested one. 
Interestingly, as our experiments revealed, for anti-diametric destinations, chosen 
routes do not include in their majority turns, because the vehicle traffic is mostly 
uniform across the road network.
